A Factor-Based Framework for Decision-Making Competency Self-Assessment

We summarize our efforts to date in developing a framework for generating succinct human-understandable competency self-assessments in terms of machine self confidence, i.e. a robot's self-trust in its functional abilities to accomplish assigned tasks. Whereas early work explored machine self-confidence in ad hoc ways for niche applications, our Factorized Machine Self-Confidence framework introduces and combines several aspects of probabilistic meta reasoning for algorithmic planning and decision-making under uncertainty to arrive at a novel set of generalizable self-confidence factors, which can support competency assessment for a wide variety of problems.

==> AAAI SS -- Proficiency/FaMSeC_math_commands.tex <==
%%%%% FaMSeC Math shortcut commands
% try to make this file somewhat `self-sustaining' so we can 
% use it in other places
\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{bm}

\DeclareMathOperator*{\argmax}{\arg\!\max}

\newcommand{\famsec}{FaMSeC}
\newcommand{\solve}{\ensuremath{\mathcal{S}}}
\newcommand{\solveopt}{\ensuremath{\mathcal{S}^*}}
\newcommand{\solvecand}{\ensuremath{\mathcal{S}^C}}
\newcommand{\solvetrust}{\ensuremath{\mathcal{S}^T}}
\newcommand{\taskclass}{\ensuremath{c_{\mathcal{T}}}}
\newcommand{\task}{\ensuremath{\mathcal{T}}}
\newcommand{\taski}{\ensuremath{\mathcal{T}_i}}
\newcommand{\taskN}{\ensuremath{\mathcal{T}_N}}
\newcommand{\rwd}{\ensuremath{\mathcal{R}}}
\newcommand{\rwdopt}{\ensuremath{\mathcal{R}^*}}
\newcommand{\rwdoptapprox}{\ensuremath{\widetilde{\mathcal{R}}^*}}
\newcommand{\rwdapprox}{\ensuremath{\widetilde{\mathcal{R}}}}
\newcommand{\rwdpredicted}{\ensuremath{\hat{\mathcal{R}}}}
\newcommand{\rwdcand}{\ensuremath{\mathcal{R}^C}}
\newcommand{\rwdcandsim}{\ensuremath{\widetilde{\mathcal{R}}^C}}
\newcommand{\rwdtrust}{\ensuremath{\mathcal{R}^T}}
\newcommand{\rwdtrusti}{\ensuremath{\mathcal{R}^T_i}}
\newcommand{\rwdtrustN}{\ensuremath{\mathcal{R}^T_N}}
\newcommand{\rwdtrustpredict}{\ensuremath{\hat{\mathcal{R}}^T}}
\newcommand{\rwdtrustipredict}{\ensuremath{\hat{\mathcal{R}}^T_i}}
\newcommand{\rwdtrustisim}{\ensuremath{\widetilde{\mathcal{R}}^T_i}}
\newcommand{\policy}{\ensuremath{\mathcal{\pi}}}
\newcommand{\policyopt}{\ensuremath{\mathcal{\pi^*}}}
\newcommand{\policytrust}{\ensuremath{\mathcal{\pi}^T}}
\newcommand{\policycand}{\ensuremath{\mathcal{\pi}^C}}
\newcommand{\surrogate}{\ensuremath{\mathcal{M}(\mathcal{T})}}
\newcommand{\surrogatearg}[1]{\ensuremath{\mathcal{M}(#1)}}
\newcommand{\xQ}{\ensuremath{x_Q}} %solver quality
\newcommand{\xO}{\ensuremath{x_O}} %outcome assessment
\newcommand{\xP}{\ensuremath{x_P}} %past performance
\newcommand{\xI}{\ensuremath{x_I}} %command interpretation
\newcommand{\xM}{\ensuremath{x_M}} %model validity
\newcommand{\xind}{\ensuremath{x_i}} % generic factor, would use \xi but it is taken
\newcommand{\xSC}{\ensuremath{x_{SC}} = \{\xI, \xM, \xQ, \xO, \xP \}}
\newcommand{\dkl}{\ensuremath{D_{KL}}}
\newcommand{\hell}{\ensuremath{H^2}}
\newcommand{\hellmet}{\ensuremath{\hell(P,Q)}}
\newcommand{\dmu}{\ensuremath{\Delta \mu}}
\def\-{\raisebox{.75pt}{-}} %short negative sign
\newcommand{\ri}{\ensuremath{R_{\infty}}}
\newcommand{\riref}{\ensuremath{\bar{R}_{\infty}}}
\newcommand{\pigeneric}{\ensuremath{\pi}}
\newcommand{\piapprox}{\ensuremath{\tilde{\pi}}}
\newcommand{\piopt}{\ensuremath{\pi^*}}
\newcommand{\picand}{\ensuremath{\pi^C}}
\newcommand{\pitrust}{\ensuremath{\pi^T}}
\newcommand{\pri}{\ensuremath{p(\ri)}}
\newcommand{\ppioptri}{\ensuremath{p_{\pi^*}(\ri)}}
\newcommand{\ppigenericri}{\ensuremath{p_{\tilde{\pi}}(R_{\infty})}}
\newcommand{\ppitrustpredict}{\ensuremath{\hat{p}_{\pi^T}(R_{\infty})}}
\newcommand{\ppicand}{\ensuremath{p_{\pi^C}(R_{\infty})}}
\newcommand{\ps}[1]{\ensuremath{p<#1}}
\newcommand{\pns}{\ensuremath{p>0.05}}
\newcommand{\cd}[1]{\ensuremath{d=#1}}
\newcommand{\Fratio}[4]{\ensuremath{(F_{#1,#2}=#3,\ps{#4})}}
\newcommand{\FratioCohen}[5]{\ensuremath{(F_{#1,#2}=#3,\ps{#4},\cd{#5})}}
\newcommand{\Frations}[3]{\ensuremath{(F_{#1,#2}=#3,\pns{})}}
\newcommand{\MSD}[2]{\ensuremath{(M=#1,SD=#2)}}
\newcommand{\CMSD}[3]{\ensuremath{(}Condition: #1;\ensuremath{M=#2,SD=#3)}}
\newcommand{\xQRR}{\ensuremath{\xQ(\rwdtrustpredict,\rwdcandsim)}}
\newcommand{\lwr}[1]{\ensuremath{L_{#1}}}
\newcommand{\upr}[1]{\ensuremath{U_{#1}}}
\newcommand{\flow}{\ensuremath{\lwr{\xind}}}
\newcommand{\fup}{\ensuremath{\upr{\xind}}}
\newcommand{\xMlow}{\ensuremath{\lwr{\xM}}}
\newcommand{\xMup}{\ensuremath{\upr{\xM}}}
\newcommand{\xIlow}{\ensuremath{\lwr{\xI}}}
\newcommand{\xIup}{\ensuremath{\upr{\xI}}}
\newcommand{\xPlow}{\ensuremath{\lwr{\xP}}}
\newcommand{\xPup}{\ensuremath{\upr{\xP}}}
\newcommand{\xQlow}{\ensuremath{\lwr{\xQ}}}
\newcommand{\xQup}{\ensuremath{\upr{\xQ}}}
\newcommand{\Upolicyopts}{\ensuremath{U^{*}(s)}}
\newcommand{\piopts}{\ensuremath{\piopt(s)}}
\newcommand{\emcts}{\ensuremath{e_{mcts}}}
\newcommand{\dmcts}{\ensuremath{d_{mcts}}}
\newcommand{\itsmcts}{\ensuremath{its_{mcts}}}
\newcommand{\rwdexit}{\ensuremath{rwd_{exit}}}
\newcommand{\rwdcaught}{\ensuremath{rwd_{caught}}}
\newcommand{\rwdsense}{\ensuremath{rwd_{sense}}}

